Quadratic Objective Perturbation: Curvature-Based Differential Privacy

Objective perturbation is a standard mechanism in differentially private empirical risk minimization. In particular, Linear Objective Perturbation (LOP) enforces privacy by adding a random linear term, while strong convexity and stability are ensured by an additional deterministic quadratic term. However, this approach requires the strong assumption of bounded gradients of the loss function, which excludes many modern machine learning models. In this work, we introduce Quadratic Objective Perturbation (QOP), which perturbs the objective with a random quadratic form. This perturbation induces strong convexity and enforces stability of the problem through curvature, thereby enabling privacy and allowing sensitivity to be controlled through spectral properties of the perturbation rather than assumptions on the gradients. As a result, we obtain $(\varepsilon, \delta)$-differential privacy under weaker \red{gradient} assumptions. Furthermore, we extend the analysis to account for approximate solutions, showing that privacy guarantees are preserved under inexact solves. Additionally, we derive utility guarantees in terms of empirical excess risk, and provide a theoretical and numerical comparison to LOP, highlighting the advantages of curvature-based perturbations. Finally, we discuss algorithmic aspects and show that the resulting problems can be solved efficiently using modern splitting schemes.

==> customcommands.tex <==
% --- Packages ---                       % Set margins
\usepackage{parskip}                % Removes indent at start of paragraph
\usepackage[scale=2]{ccicons}
\usepackage{booktabs}
\usepackage{amsmath}
\usepackage{amssymb}            
\usepackage{graphicx}               % To import pictures
\usepackage{mathtools}              % Allows various math, such as \coloneqq
\usepackage{multicol, multirow}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{array}
\usepackage{tikz}                   % For Tikz figures
\usepackage{pgfplots}               % For PGF figures, makes Tikz easier
\pgfplotsset{compat=newest}
\usepackage{xcolor}                 % For colors
\usepackage{natbib}                 % For citations
\usepackage{bibentry}               % For bibtex entries
\usepackage[normalem]{ulem}         % For strikeout using \sout
\usepackage{tablefootnote}          % For footnotes in tables

% --- Hyperref setup ---
\usepackage[breaklinks, colorlinks=true]{hyperref}
\definecolor{lessred}{HTML}{FF5010} 
\definecolor{lessblue}{HTML}{4BAAC8} 
\definecolor{lessgreen}{HTML}{AA10AA} 
\hypersetup{
    colorlinks=true,
    linkcolor=lessred,
    filecolor=magenta,      
    urlcolor=magenta,
    citecolor=lessblue
    }

% --- Custom commands ---
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{\mathbb{P}}
\renewcommand{\H}{\mathcal{H}}

\newcommand{\Var}{\operatorname{Var}}
\newcommand{\argmin}{\operatorname{argmin}}
\newcommand{\prox}{\operatorname{prox}}
\newcommand{\proj}{\operatorname{proj}}
\newcommand{\cone}{\operatorname{cone}}
\newcommand{\interior}{\operatorname{int}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\spa}{\operatorname{span}}
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\Zer}{\operatorname{Zer}}
\newcommand{\diam}{\operatorname{diam}}

% Specific to PIKM Project
\newcommand{\Fix}{\operatorname{Fix}}

% Specific to SGD Project
\newcommand{\Exp}[1]{\mathbb{E}\mathopen{}\left[{#1}\right]\mathclose{}}
\newcommand{\Expt}[1]{\mathbb{E}_t\mathopen{}\left[{#1}\right]\mathclose{}}
\newcommand{\ExpD}[2]{\mathbb{E}_{{#1}}\mathopen{}\left[{#2}\right]\mathclose{}}

% Specific to HVI Project
\newcommand{\Gap}[1]{\operatorname{Gap}({#1})}
\newcommand{\GapOpt}[1]{\operatorname{Gap}_{\operatorname{opt}}({#1})}
\newcommand{\GapFeas}[1]{\operatorname{Gap}_{\operatorname{feas}}({#1})}

% Specific to SKM Project
\newcommand{\supp}{\operatorname{supp}}
\renewcommand{\O}{{\mathcal O}}
\newcommand{\graph}{\operatorname{graph}}

% Specific to DP Project
\newcommand{\D}{{\mathcal D}}
\renewcommand{\L}{{\mathcal L}}
\renewcommand{\S}{{\mathbb S}}
\newcommand{\X}{{\mathcal X}}
\newcommand{\priv}{{\operatorname{priv}}}
\newcommand{\Wishart}{{\operatorname{Wishart}}}
\newcommand{\sym}{{\operatorname{sym}}}
\newcommand{\rank}{{\operatorname{rank}}}
\newcommand{\exact}{{\operatorname{ex}}}
\newcommand{\final}{{\operatorname{final}}}
\newcommand{\Jp}{{\mathcal J_\priv}}
\newcommand{\Jpi}{{\mathcal J_\priv^i}}
\newcommand{\tJp}{{\widetilde{\mathcal J}_\priv}}
\newcommand{\J}{{\mathcal J}}
\newcommand{\ran}{\operatorname{ran}}
\newcommand{\op}{\operatorname{op}}
\newcommand{\lin}{{\operatorname{lin}}}

% Specific to CNM Project
\newcommand{\slow}{{\operatorname{slow}}}
\newcommand{\fast}{{\operatorname{fast}}}

% --- Tick and cross marks from pifont ---
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}

% --- Commenting ---
\newcommand{\red}[1]{{\color{red}{{#1}}}}
\newcommand{\DC}[1]{{\color{red}{[\textbf{DC}: {#1}]}}}
\setlength{\marginparwidth}{2cm}
\usepackage[colorinlistoftodos,bordercolor=orange,backgroundcolor=orange!20,linecolor=orange]{todonotes}
\newcommand{\daniel}[1]{\todo[inline]{\textbf{Daniel: }#1}}

% --- For Tables ---
\usepackage{tabularx}
\usepackage{array}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}

% --- For Citations within Theorem Names ---
\newcommand{\thmcite}[2][]{%
  \citeauthor{#2}, \citeyear{#2}%
  \if\relax\detokenize{#1}\relax
    % optional arg empty -> do nothing
  \else
    , #1%
  \fi
}

% --- For Papers that are moved to other files ---
\usepackage{draftwatermark}
\SetWatermarkText{}
\newcommand{\moved}{
    \SetWatermarkText{- DRAFT - \\ MOVED TO \\ OTHER FILE}
    \SetWatermarkScale{4}        % size (adjust as needed)
    \SetWatermarkColor[gray]{0.7} % light gray (default style)
}

% --- Remove space around \left and \right ---
\usepackage{mleftright}
\renewcommand{\left}{\mleft}
\renewcommand{\right}{\mright}

% --- Orcid Repertoire ---
\usepackage{orcidlink}              % For ORCID Links
\newcommand{\orcidCortild}{\orcidlink{0000-0002-3278-1716} }
\newcommand{\orcidCartis}{\orcidlink{0000-0002-0963-5550} }

% --- Add line numbers fo review ---
\usepackage{lineno}
\newcommand{\review}{\linenumbers}

% --- Nicer Bibtex ---

